ContextQ: Generated Questions to Support Meaningful Parent-Child Dialogue While Co-Reading

Much of early literacy education happens at home with caretakers reading books to young children. Prior research demonstrates how having dialogue with children during co-reading can develop critical reading readiness skills, but most adult readers are unsure if and how to lead effective conversations. We present ContextQ, a tablet-based reading application to unobtrusively present auto-generated dialogic questions to caretakers to support this dialogic reading practice. An ablation study demonstrates how our method of encoding educator expertise into the question generation pipeline can produce high-quality output; and through a user study with 12 parent-child dyads (child age: 4-6), we demonstrate that this system can serve as a guide for parents in leading contextually meaningful dialogue, leading to significantly more conversational turns from both the parent and the child and deeper conversations with connections to the child's everyday life.

==> references.tex <==
@article{hernandez2011double,
  title={Double jeopardy: How third-grade reading skills and poverty influence high school graduation.},
  author={Hernandez, Donald J},
  journal={Annie E. Casey Foundation},
  year={2011},
  publisher={ERIC}
}

@book{boyer1991ready,
  title={Ready to learn: A mandate for the nation},
  author={Boyer, Ernest L and Carnegie Foundation for the Advancement of Teaching (Princeton NJ)},
  year={1991},
  publisher={Carnegie Foundation for the Advancement of Teaching Princeton, NJ}
}

@article{krcmar2014parent,
  title={Parent--child joint reading in traditional and electronic formats},
  author={Krcmar, Marina and Cingel, Drew P},
  journal={Media Psychology},
  volume={17},
  number={3},
  pages={262--281},
  year={2014},
  publisher={Taylor \& Francis}
}

@article{zevenbergen2003dialogic,
  title={Dialogic reading: A shared picture book reading intervention for preschoolers},
  author={Zevenbergen, Andrea A and Whitehurst, Grover J},
  journal={On reading books to children: Parents and teachers},
  volume={177},
  pages={200},
  year={2003}
}

@article{zimmerman2009teaching,
  title={Teaching by listening: The importance of adult-child conversations to language development},
  author={Zimmerman, Frederick J and Gilkerson, Jill and Richards, Jeffrey A and Christakis, Dimitri A and Xu, Dongxin and Gray, Sharmistha and Yapanel, Umit},
  journal={Pediatrics},
  volume={124},
  number={1},
  pages={342--349},
  year={2009},
  publisher={American Academy of Pediatrics}
}

@article{troseth2020enhanced,
  title={An enhanced eBook facilitates parent--child talk during shared reading by families of low socioeconomic status},
  author={Troseth, Georgene L and Strouse, Gabrielle A and Flores, Israel and Stuckelman, Zachary D and Johnson, Colleen Russo},
  journal={Early childhood research quarterly},
  volume={50},
  pages={45--58},
  year={2020},
  publisher={Elsevier}
}

@article{doyle2006promoting,
  title={Promoting emergent literacy and social--emotional learning through dialogic reading},
  author={Doyle, Brooke Graham and Bramwell, Wendie},
  journal={The Reading Teacher},
  volume={59},
  number={6},
  pages={554--564},
  year={2006},
  publisher={Wiley Online Library}
}

@article{stuckelman2021value,
  title={Value added: Digital modeling of dialogic questioning promotes positive parenting during shared reading.},
  author={Stuckelman, Zachary D and Strouse, Gabrielle A and Troseth, Georgene L},
  journal={Journal of Family Psychology},
  year={2021},
  publisher={American Psychological Association}
}

@inproceedings{zhang2022storybuddy,
  title={StoryBuddy: A Human-AI Collaborative Chatbot for Parent-Child Interactive Storytelling with Flexible Parental Involvement},
  author={Zhang, Zheng and Xu, Ying and Wang, Yanhao and Yao, Bingsheng and Ritchie, Daniel and Wu, Tongshuang and Yu, Mo and Wang, Dakuo and Li, Toby Jia-Jun},
  booktitle={CHI Conference on Human Factors in Computing Systems},
  pages={1--21},
  year={2022}
}

@article{whitehurst1988accelerating,
  title={Accelerating language development through picture book reading.},
  author={Whitehurst, Grover J and Falco, Francine L and Lonigan, Christopher J and Fischel, Janet E and DeBaryshe, Barbara D and Valdez-Menchaca, Marta C and Caulfield, Marie},
  volume={24},
  number={4},
  pages={552},
  year={1988},
  publisher={American Psychological Association}
}

@article{valdez1992accelerating,
  title={Accelerating language development through picture book reading: A systematic extension to Mexican day care.},
  author={Valdez-Menchaca, Marta C and Whitehurst, Grover J},
  journal={Developmental psychology},
  volume={28},
  number={6},
  pages={1106},
  year={1992},
  publisher={American Psychological Association}
}

@article{arnold1994accelerating,
  title={Accelerating language development through picture book reading: replication and extension to a videotape training format.},
  author={Arnold, David H and Lonigan, Christopher J and Whitehurst, Grover J and Epstein, Jeffery N},
  journal={Journal of educational psychology},
  volume={86},
  number={2},
  pages={235},
  year={1994},
  publisher={American Psychological Association}
}

@article{lim2002facilitating,
  title={Facilitating first language development in young Korean children through parent training in picture book interactions},
  author={Lim, Young Sook and Cole, Kevin N},
  journal={Bilingual Research Journal},
  volume={26},
  number={2},
  pages={367--381},
  year={2002},
  publisher={Taylor \& Francis}
}

@book{boyatzis98,
    author = {Boyatzis, Richard E},
    title = {Transforming Qualitative Information: Thematic Analysis and Code Development},
    publisher = {Sage Publications} ,
    year = {1998}
}


@article{flynn2011,
    author = {Kylie S. Flynn},
    title ={Developing Children's Oral Language Skills through Dialogic Reading: Guidelines for Implementation},
    journal = {TEACHING Exceptional Children},
    volume = {44},
    number = {2},
    pages = {8-16},
    year = {2011},
    doi = {10.1177/004005991104400201},
    URL = { 
            https://doi.org/10.1177/004005991104400201
    },
    eprint = { 
            https://doi.org/10.1177/004005991104400201   
    }
}

@article{cegis,
author = {Solar-Lezama, Armando and Tancau, Liviu and Bodik, Rastislav and Seshia, Sanjit and Saraswat, Vijay},
title = {Combinatorial Sketching for Finite Programs},
year = {2006},
issue_date = {December 2006},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {34},
number = {5},
issn = {0163-5964},
url = {https://doi.org/10.1145/1168919.1168907},
doi = {10.1145/1168919.1168907},
abstract = {Sketching is a software synthesis approach where the programmer develops a partial implementation - a sketch - and a separate specification of the desired functionality. The synthesizer then completes the sketch to behave like the specification. The correctness of the synthesized implementation is guaranteed by the compiler, which allows, among other benefits, rapid development of highly tuned implementations without the fear of introducing bugs.We develop SKETCH, a language for finite programs with linguistic support for sketching. Finite programs include many highperformance kernels, including cryptocodes. In contrast to prior synthesizers, which had to be equipped with domain-specific rules, SKETCH completes sketches by means of a combinatorial search based on generalized boolean satisfiability. Consequently, our combinatorial synthesizer is complete for the class of finite programs: it is guaranteed to complete any sketch in theory, and in practice has scaled to realistic programming problems.Freed from domain rules, we can now write sketches as simpleto-understand partial programs, which are regular programs in which difficult code fragments are replaced with holes to be filled by the synthesizer. Holes may stand for index expressions, lookup tables, or bitmasks, but the programmer can easily define new kinds of holes using a single versatile synthesis operator.We have used SKETCH to synthesize an efficient implementation of the AES cipher standard. The synthesizer produces the most complex part of the implementation and runs in about an hour.},
journal = {SIGARCH Comput. Archit. News},
month = {oct},
pages = {404–415},
numpages = {12},
keywords = {sketching, SAT}
}

@inproceedings{Xiao_2023,
	doi = {10.1145/3581754.3584136},
	url = {https://doi.org/10.1145%2F3581754.3584136},
	year = 2023,
	month = {mar},
	publisher = {{ACM}
},
	author = {Ziang Xiao and Xingdi Yuan and Q. Vera Liao and Rania Abdelghani and Pierre-Yves Oudeyer},
	title = {Supporting Qualitative Analysis with Large Language Models: Combining Codebook with {GPT}-3 for Deductive Coding},
	booktitle = {28th International Conference on Intelligent User Interfaces}
}


@misc{liu2021pretrain,
      title={Pre-train, Prompt, and Predict: A Systematic Survey of Prompting Methods in Natural Language Processing}, 
      author={Pengfei Liu and Weizhe Yuan and Jinlan Fu and Zhengbao Jiang and Hiroaki Hayashi and Graham Neubig},
      year={2021},
      eprint={2107.13586},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}


@article{Schaffalitzky2022WhatMA,
  title={What makes authentic questions authentic?},
  author={Caroline Schaffalitzky},
  journal={Dialogic Pedagogy: An International Online Journal},
  year={2022}
}

@article{nystrand2003questions,
  title={Questions in time: Investigating the structure and dynamics of unfolding classroom discourse},
  author={Nystrand, Martin and Wu, Lawrence L and Gamoran, Adam and Zeiser, Susie and Long, Daniel A},
  journal={Discourse processes},
  volume={35},
  number={2},
  pages={135--198},
  year={2003},
  publisher={Taylor \& Francis}
}

@InProceedings{CevskaProbCEGIS,
author="{\v{C}}e{\v{s}}ka, Milan
and Hensel, Christian
and Junges, Sebastian
and Katoen, Joost-Pieter",
editor="ter Beek, Maurice H.
and McIver, Annabelle
and Oliveira, Jos{\'e} N.",
title="Counterexample-Driven Synthesis for Probabilistic Program Sketches",
booktitle="Formal Methods -- The Next 30 Years",
year="2019",
publisher="Springer International Publishing",
address="Cham",
pages="101--120",
abstract="Probabilistic programs are key to deal with uncertainty in, e.g., controller synthesis. They are typically small but intricate. Their development is complex and error prone requiring quantitative reasoning over a myriad of alternative designs. To mitigate this complexity, we adopt counterexample-guided inductive synthesis (CEGIS) to automatically synthesise finite-state probabilistic programs. Our approach leverages efficient model checking, modern SMT solving, and counterexample generation at program level. Experiments on practically relevant case studies show that design spaces with millions of candidate designs can be fully explored using a few thousand verification queries.",
isbn="978-3-030-30942-8"
}



@article{gunby2011,
author = {Jessica T. DeCuir-Gunby and Patricia L. Marshall and Allison W. McCulloch},
title ={Developing and Using a Codebook for the Analysis of Interview Data: An Example from a Professional Development Research Project},
journal = {Field Methods},
volume = {23},
number = {2},
pages = {136-155},
year = {2011},
doi = {10.1177/1525822X10388468},

URL = { 
        https://doi.org/10.1177/1525822X10388468
    
},
eprint = { 
        https://doi.org/10.1177/1525822X10388468
    
}
,
    abstract = { This article gives specific steps on how to create a codebook for coding interview data. The authors examine the development of theory- and data-driven codes through the discussion of a professional development (PD) research project. They also discuss how to train others to code using the codebook, including how to establish reliability. The authors end with practical suggestions from their experiences in creating a codebook. }
}

@book{Nystrand_1997, place={New York}, title={Opening dialogue: Understanding the dynamics of language and learning in the English classroom}, publisher={Teachers College Press}, author={Nystrand, Martin}, year={1997}} 


@inbook{Costa_2001, place={Alexandria, VA}, title={Toward a Model of Human Intellectual Functioning},
booktitle={Developing minds: A resource book for teaching thinking}, publisher={Association for Supervision and Curriculum Development}, author={Costa, Arthur L.}, year={2001}} 

@book{costa1989techniques,
  title={Techniques for teaching thinking},
  author={Costa, Arthur and Lowery, Lawrence F},
  year={1989},
  publisher={Routledge}
}


@book{bloom1956taxonomy,
  title = {Taxonomy of Educational Objectives: The Classification of Educational Goals. Handbook I: Cognitive Domain},
  author = {Bloom, Benjamin S.},
  year = {1956},
  publisher = {David McKay Company},
  address = {New York},
}

@inproceedings{raffle2011hello,
  title={Hello, is grandma there? let's read! StoryVisit: family video chat and connected e-books},
  author={Raffle, Hayes and Revelle, Glenda and Mori, Koichi and Ballagas, Rafael and Buza, Kyle and Horii, Hiroshi and Kaye, Joseph and Cook, Kristin and Freed, Natalie and Go, Janet and others},
  booktitle={Proceedings of the SIGCHI conference on human factors in computing systems},
  pages={1195--1204},
  year={2011}
}

@article{whitehurst1994outcomes,
  title={Outcomes of an emergent literacy intervention in Head Start.},
  author={Whitehurst, Grover J and Epstein, Jeffrey N and Angell, Andrea L and Payne, Adam C and Crone, Deanne A and Fischel, Janet E},
  journal={Journal of Educational Psychology},
  volume={86},
  number={4},
  pages={542},
  year={1994},
  publisher={American Psychological Association}
}

@article{mol2008added,
  title={Added value of dialogic parent--child book readings: A meta-analysis},
  author={Mol, Suzanne E and Bus, Adriana G and De Jong, Maria T and Smeets, Daisy JH},
  journal={Early education and development},
  volume={19},
  number={1},
  pages={7--26},
  year={2008},
  publisher={Taylor \& Francis}
}

@article{hindman2016closing,
  title={Closing the 30 million word gap: Next steps in designing research to inform practice},
  author={Hindman, Annemarie H and Wasik, Barbara A and Snell, Emily K},
  journal={Child Development Perspectives},
  volume={10},
  number={2},
  pages={134--139},
  year={2016},
  publisher={Wiley Online Library}
}

@article{strouse2013effective,
  title={Effective coviewing: Preschoolers’ learning from video after a dialogic questioning intervention.},
  author={Strouse, Gabrielle A and O'Doherty, Katherine and Troseth, Georgene L},
  journal={Developmental psychology},
  volume={49},
  number={12},
  pages={2368},
  year={2013},
  publisher={American Psychological Association}
}

@article{korat2010new,
  title={How new technology influences parent—child interaction: The case of e-book reading},
  author={Korat, Ofra and Or, Tal},
  journal={First Language},
  volume={30},
  number={2},
  pages={139--154},
  year={2010},
  publisher={Sage Publications Sage UK: London, England}
}

@article{korngiebel2021considering,
  title={Considering the possibilities and pitfalls of Generative Pre-trained Transformer 3 (GPT-3) in healthcare delivery},
  author={Korngiebel, Diane M and Mooney, Sean D},
  journal={NPJ Digital Medicine},
  volume={4},
  number={1},
  pages={93},
  year={2021},
  publisher={Nature Publishing Group UK London}
}

@inproceedings{xu2023rosita,
  title={“Rosita Reads With My Family”: Developing A Bilingual Conversational Agent to Support Parent-Child Shared Reading},
  author={Xu, Ying and He, Kunlei and Vigil, Valery and Ojeda-Ramirez, Santiago and Liu, Xuechen and Levine, Julian and Cervera, Kelsyann and Warschauer, Mark},
  booktitle={Proceedings of the 22nd Annual ACM Interaction Design and Children Conference},
  pages={160--172},
  year={2023}
}

@inproceedings{curto2011exploring,
  title={Exploring linguistically-rich patterns for question generation},
  author={Curto, S{\'e}rgio and Mendes, Ana Cristina and Coheur, Lu{\'\i}sa},
  booktitle={Proceedings of the UCNLG+ eval: Language Generation and Evaluation Workshop},
  pages={33--38},
  year={2011}
}

@inproceedings{labutov2015deep,
  title={Deep questions without deep understanding},
  author={Labutov, Igor and Basu, Sumit and Vanderwende, Lucy},
  booktitle={Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  pages={889--898},
  year={2015}
}

@article{du2017learning,
  title={Learning to ask: Neural question generation for reading comprehension},
  author={Du, Xinya and Shao, Junru and Cardie, Claire},
  journal={arXiv preprint arXiv:1705.00106},
  year={2017}
}

@article{dong2019unified,
  title={Unified language model pre-training for natural language understanding and generation},
  author={Dong, Li and Yang, Nan and Wang, Wenhui and Wei, Furu and Liu, Xiaodong and Wang, Yu and Gao, Jianfeng and Zhou, Ming and Hon, Hsiao-Wuen},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@article{tang2017question,
  title={Question answering and question generation as dual tasks},
  author={Tang, Duyu and Duan, Nan and Qin, Tao and Yan, Zhao and Zhou, Ming},
  journal={arXiv preprint arXiv:1706.02027},
  year={2017}
}

@article{yao2021ai,
  title={It is AI's Turn to Ask Humans a Question: Question-Answer Pair Generation for Children's Story Books},
  author={Yao, Bingsheng and Wang, Dakuo and Wu, Tongshuang and Zhang, Zheng and Li, Toby Jia-Jun and Yu, Mo and Xu, Ying},
  journal={arXiv preprint arXiv:2109.03423},
  year={2021}
}

@article{choi2018quac,
  title={QuAC: Question answering in context},
  author={Choi, Eunsol and He, He and Iyyer, Mohit and Yatskar, Mark and Yih, Wen-tau and Choi, Yejin and Liang, Percy and Zettlemoyer, Luke},
  journal={arXiv preprint arXiv:1808.07036},
  year={2018}
}

@article{francis1996developmental,
  title={Developmental lag versus deficit models of reading disability: A longitudinal, individual growth curves analysis.},
  author={Francis, David J and Shaywitz, Sally E and Stuebing, Karla K and Shaywitz, Bennett A and Fletcher, Jack M},
  journal={Journal of Educational psychology},
  volume={88},
  number={1},
  pages={3},
  year={1996},
  publisher={American Psychological Association}
}

@article{juel1988learning,
  title={Learning to read and write: A longitudinal study of 54 children from first through fourth grades.},
  author={Juel, Connie},
  journal={Journal of educational Psychology},
  volume={80},
  number={4},
  pages={437},
  year={1988},
  publisher={American Psychological Association}
}

@article{torgesen1998consistency,
  title={Consistency of reading-related phonological processes throughout early childhood: Evidence from longitudinal-correlational and instructional studies},
  author={Torgesen, Joseph K and Burgess, Stephen R},
  journal={Word recognition in beginning literacy},
  volume={161},
  pages={188},
  year={1998}
}

@article{bommasani2021opportunities,
  title={On the opportunities and risks of foundation models},
  author={Bommasani, Rishi and Hudson, Drew A and Adeli, Ehsan and Altman, Russ and Arora, Simran and von Arx, Sydney and Bernstein, Michael S and Bohg, Jeannette and Bosselut, Antoine and Brunskill, Emma and others},
  journal={arXiv preprint arXiv:2108.07258},
  year={2021}
}

@article{vasileiadou2021examining,
  title={Examining the impact of self-assessment with the use of rubrics on primary school students’ performance},
  author={Vasileiadou, Despina and Karadimitriou, Konstantinos},
  journal={International Journal of Educational Research Open},
  volume={2},
  pages={100031},
  year={2021},
  publisher={Elsevier}
}

@article{andrade2000using,
  title={Using rubrics to promote thinking and learning},
  author={Andrade, Heidi Goodrich},
  journal={Educational leadership},
  volume={57},
  number={5},
  pages={13--19},
  year={2000},
  publisher={Citeseer}
}

@article{sundeen2014instructional,
  title={Instructional rubrics: Effects of presentation options on writing quality},
  author={Sundeen, Todd H},
  journal={Assessing writing},
  volume={21},
  pages={74--88},
  year={2014},
  publisher={Elsevier}
}

@book{goodrich1996student,
  title={Student self-assessment: At the intersection of metacognition and authentic assessment},
  author={Goodrich, Heidi Watts},
  year={1996},
  publisher={Harvard University}
}

@article{kim2023prometheus,
  title={Prometheus: Inducing Fine-grained Evaluation Capability in Language Models},
  author={Kim, Seungone and Shin, Jamin and Cho, Yejin and Jang, Joel and Longpre, Shayne and Lee, Hwaran and Yun, Sangdoo and Shin, Seongjin and Kim, Sungdong and Thorne, James and others},
  journal={arXiv preprint arXiv:2310.08491},
  year={2023}
}

@inproceedings{markov2023holistic,
  title={A holistic approach to undesired content detection in the real world},
  author={Markov, Todor and Zhang, Chong and Agarwal, Sandhini and Nekoul, Florentine Eloundou and Lee, Theodore and Adler, Steven and Jiang, Angela and Weng, Lilian},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={37},
  number={12},
  pages={15009--15018},
  year={2023}
}

@article{rebedea2023nemo,
  title={Nemo guardrails: A toolkit for controllable and safe llm applications with programmable rails},
  author={Rebedea, Traian and Dinu, Razvan and Sreedhar, Makesh and Parisien, Christopher and Cohen, Jonathan},
  journal={arXiv preprint arXiv:2310.10501},
  year={2023}
}

@article{goodfellow2020generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Communications of the ACM},
  volume={63},
  number={11},
  pages={139--144},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{sherin2013computational,
  title={A computational study of commonsense science: An exploration in the automated analysis of clinical interview data},
  author={Sherin, Bruce},
  journal={Journal of the Learning Sciences},
  volume={22},
  number={4},
  pages={600--638},
  year={2013},
  publisher={Taylor \& Francis}
}

@article{beck2001text,
  title={Text talk: Capturing the benefits of read-aloud experiences for young children},
  author={Beck, Isabel L and McKeown, Margaret G},
  journal={The reading teacher},
  volume={55},
  number={1},
  pages={10--20},
  year={2001},
  publisher={JSTOR}
}

@article{duursma2008reading,
  title={Reading aloud to children: the evidence},
  author={Duursma, Elisabeth and Augustyn, Marilyn and Zuckerman, Barry},
  journal={Archives of disease in childhood},
  volume={93},
  number={7},
  pages={554--557},
  year={2008},
  publisher={BMJ Publishing Group Ltd}
}

@article{braun2006using,
  title={Using thematic analysis in psychology},
  author={Braun, Virginia and Clarke, Victoria},
  journal={Qualitative research in psychology},
  volume={3},
  number={2},
  pages={77--101},
  year={2006},
  publisher={Taylor \& Francis}
}

@inproceedings{bacchelli2013expectations,
  title={Expectations, outcomes, and challenges of modern code review},
  author={Bacchelli, Alberto and Bird, Christian},
  booktitle={2013 35th International Conference on Software Engineering (ICSE)},
  pages={712--721},
  year={2013},
  organization={IEEE}
}

@inproceedings{kononenko2016code,
  title={Code review quality: How developers see it},
  author={Kononenko, Oleksii and Baysal, Olga and Godfrey, Michael W},
  booktitle={Proceedings of the 38th international conference on software engineering},
  pages={1028--1038},
  year={2016}
}

@inproceedings{sadowski2018modern,
  title={Modern code review: a case study at google},
  author={Sadowski, Caitlin and S{\"o}derberg, Emma and Church, Luke and Sipko, Michal and Bacchelli, Alberto},
  booktitle={Proceedings of the 40th international conference on software engineering: Software engineering in practice},
  pages={181--190},
  year={2018}
}

@article{xu2022fantastic,
  title={Fantastic Questions and Where to Find Them: FairytaleQA--An Authentic Dataset for Narrative Comprehension},
  author={Xu, Ying and Wang, Dakuo and Yu, Mo and Ritchie, Daniel and Yao, Bingsheng and Wu, Tongshuang and Zhang, Zheng and Li, Toby Jia-Jun and Bradford, Nora and Sun, Branda and others},
  journal={arXiv preprint arXiv:2203.13947},
  year={2022}
}

@article{leech2021intervention,
  title={An intervention to increase conversational turns between parents and young children},
  author={Leech, Kathryn A and others},
  journal={Journal of Child Language},
  volume={48},
  number={2},
  pages={399--412},
  year={2021},
  publisher={Cambridge University Press}
}

@article{leech2018brief,
  title={A brief parent-focused intervention to improve preschoolers’ conversational skills and school readiness.},
  author={Leech, Kathryn and Wei, Ran and Harring, Jeffrey R and Rowe, Meredith L},
  journal={Developmental psychology},
  volume={54},
  number={1},
  pages={15},
  year={2018},
  publisher={American Psychological Association}
}
